Implicit Riemannian Optimism with Applications to Min-Max Problems

We introduce a Riemannian optimistic online learning algorithm for Hadamard manifolds based on inexact implicit updates. Unlike prior work, our method can handle in-manifold constraints, and matches the best known regret bounds in the Euclidean setting with no dependence on geometric constants, like the minimum curvature. Building on this, we develop algorithms for g-convex, g-concave smooth min-max problems on Hadamard manifolds. Notably, one method nearly matches the gradient oracle complexity of the lower bound for Euclidean problems, for the first time.

==> definitions.tex <==
\usepackage{xparse}
\usepackage{xargs}

\makeatletter 
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} 
\makeatother


\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
\newcommand\linkofproof[1]{(\cref{#1})\newtarget{proof:#1}\ }

\usepackage[bb=boondox]{mathalpha} 
\newcommand{\zeros}{\mathbb{0}} 
\newcommand\Hess{\operatorname{Hess}}


\newcommand{\innp}[1]{\langle #1 \rangle}
\newcommand{\bigo}[1]{O( #1 )}
\newcommand{\bigol}[1]{O\left( #1 \right)}
\newcommand{\bigoast}[1]{O^\ast( #1 )}
\newcommand{\bigoastl}[1]{O^\ast\left( #1 \right)}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigotildel}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigomega}[1]{\newlink{def:big_o_tilde}{\Omega}( #1 )}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}

\DeclarePairedDelimiter\card{\lvert}{\rvert}    
\newcommand{\pa}[1]{\left( #1\right)} 
\newcommand{\norm}[1]{\| #1 \|} 
\newcommand{\norml}[1]{\left\| #1 \right\|} 
\newcommand{\abs}[1]{\lvert #1 \rvert} 
\DeclarePairedDelimiter\cor{\lbrack}{\rbrack}   
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}    

\newcommand*\circledaux[1]{\tikz[baseline=(char.base)]{
\node[shape=circle,draw,inner sep=0.8pt] (char) {#1};}}

\NewDocumentCommand{\circled}{m o }{%
\IfNoValueTF{#2}{\circledaux{#1}}{\stackrel{\circledaux{#1}}{#2}}%
}

\DeclareMathOperator{\supp}{supp}                       
\DeclareMathOperator*{\diag}{diag}                      
\renewcommand*{\Im}{\mathrm{Im}}                        
\newcommand*\dif{\mathrm{d}}                            
\newcommand*\Id{\mathrm{Id}}                            
\newcommand\conn{\nabla}                                
\newcommand*\tensor{\otimes}                            
\newcommand{\defi}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
\newcommand{\defiin}{\stackrel{\mathrm{\scriptscriptstyle def}}{\in}}
\newcommand*\iso{\cong}                                 
\newcommand*\fn{\operatorname}                          
\newcommand{\code}{\texttt}                             
\newcommand\deriv[1]{\frac{\mathrm{d}}{\mathrm{d}#1}}   

\renewcommand*\C{\mathbb{C}}                              
\renewcommand*\R{\mathbb{R}}                              
\newcommand*\mean[1]{\overline{#1}}                       

\let\epsilon\varepsilon



\newcommand\trans[1]{#1^\intercal}                          
\DeclareMathOperator\tr{tr}                                 
\newcommand\dual[1]{#1^\ast}                                
\newcommand\faprox{f_{\delta, L}}                           
\newcommand\gaprox{g_{\delta, L}}                           
\newcommand\Mani{\mathcal{M}}                               
\renewcommand\S{\mathbb{S}}                                 
\DeclareMathOperator\gradmani{grad}                         
\newcommand\gradexp{\tilde{\grad}}                          
\DeclareMathOperator\ad{ad}                                 
\DeclareMathOperator\Ad{Ad}                                 
\newcommand\g{\mathfrak{g}}                                 
\DeclareMathOperator{\End}{End}                             
\newcommand\adj[1]{#1^\ast}                                 
\DeclareMathOperator{\normal}{\mathcal{N}}                  
\DeclareMathOperator{\unif}{\mathcal{U}}                    
\newcommand\I{\mathrm{I}}                                   


\newcommand{\Var}[1]{\text{Var}\left[#1\right]} 
\newcommand{\Cov}[1]{\text{Cov}\left[#1\right]} 
\renewcommand{\P}[1]{\mathbb{P}\left[#1\right]} 
\newcommand{\Vart}{\text{Var}} 
\renewcommand{\E}[1]{\mathbb{E}\left[ #1 \right]} 
\newcommand{\dirich}[1]{\mathcal{E}\left( #1 \right)} 
\newcommand{\grad}{\nabla} 
\newcommand{\ones}{\mathds{1}}                           
\newcommand{\varl}{\operatorname{left}} 
\newcommand{\varr}{\operatorname{right}} 


\usepackage{pifont} 
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\yesmark}{{\color{green} \cmark}}
\newcommand{\nomark}{{\color{red} \xmark}}


\DeclareMathOperator*{\argmax}{arg\,max}                
\DeclareMathOperator*{\argmin}{arg\,min}                


\let\oldmu\mu
\renewcommand\mu{\newlink{def:strong_g_convexity_of_F}{\oldmu}}

\newcommandx*{\Lips}[1][1=, usedefault]{\newlink{def:Lipschitz_constant}{G^{#1}}}
\let\strikedL\L
\renewcommand{\L}{\newlink{def:riemannian_smoothness_constant}{L}} 




\newcommand{\RGD}{\newlink{def:acronym_riemannian_gradient_descent}{RGD}}
\newcommand{\CRGD}{\newlink{def:acronym_composite_riemannian_gradient_descent}{CRGD}}
\newcommand{\PRGD}{\newlink{def:acronym_metric_projected_riemannian_gradient_descent}{PRGD}}
\newcommand{\RPPA}{\newlink{def:acronym_riemannian_proximal_point_algorithm}{RPPA}}
\newcommand{\RIPPA}{\newlink{def:acronym_riemannian_inexact_proximal_point_algorithm}{RIPPA}}
\newcommand{\RCEGmin}{\newlink{def:acronym_rceg_min}{RCEG-min}}
\newcommand{\RCEG}{\newlink{def:acronym_rceg}{RCEG}}
\newcommand{\RIOD}{\newlink{def:acronym_riod}{\textsc{riod}}}
\newcommand{\RIODA}{\newlink{def:acronym_rioda}{\textsc{rioda}}}

\newcommand\regret[1]{\newlink{def:regret}{R_{#1}}}

\renewcommand\M{\mathcal{M}}
\renewcommand\H{\mathcal{H}}
\newcommand\NN{\newlink{def:N_open_set_in_manifold}{\mathcal{N}}}
\newcommand{\X}{\mathcal{X}}
\newcommand*\Z{\mathcal{Z}}                                
\newcommandx*{\Rmax}[1][1=, usedefault]{\newlink{def:max_distance_to_x_ast}{R_{\max}^{#1}}}
\renewcommand{\R}{\newlink{def:initial_distance}{R}}

\newcommand{\DOL}{\newlink{def:diam_in_online_learning_alg_riod}{D}}
\newcommand{\DMM}{\newlink{def:diam_in_minmax_alg_rioda}{D}}

\newcommandx*\kmin[1][1=, usedefault]{\newlink{def:minimum_sectional_curvature}{\kappa_{\min}^{#1}}}
\newcommandx*\kmax[1][1=, usedefault]{\newlink{def:maximum_sectional_curvature}{\kappa_{\max}^{#1}}}
\newcommand\Mmin{\mathcal{M}_{\operatorname{LB}}}
\newcommand\Riemmin{\newlink{def:M_manifold_with_lower_bounded_curv}{\mathcal{R}_{\operatorname{LB}}}}
\newcommand\Riem{\newlink{def:M_manifold_with_lower_bounded_curv}{\mathcal{R}_{\operatorname{LUB}}}}

\newcommand{\dist}{\newlink{def:distance}{d}}

\newcommandx*\prox[2][1=f, 2=\eta, usedefault]{\newlink{def:prox}{\operatorname{prox}_{#2#1}}}

\newcommandx*\smc[1][1=\X, usedefault]{\newlink{def:smooth_convex_class}{\mathcal{F}_{\L}(\X)}}
\newcommandx*\smsc[3][1=\X, 2=\L, 3=\mu, usedefault]{\newlink{def:smooth_strongly_convex_class}{\mathcal{F}_{#3, #2}(#1)}}
\newcommandx*\nsmc[1][1=\X, usedefault]{\newlink{def:non_smooth_convex_class}{\mathcal{F}_{\Lips}^p(#1)}}
\newcommandx*\proxc[1][1=\M, usedefault]{\newlink{def:proper_lsc_convex_class}{\mathcal{F}(#1)}}

\newcommand{\diam}{\operatorname{diam}}
 
\newcommand\ball{\newlink{def:closed_ball}{\bar{B}}}

\newcommand\xast{\newlink{def:optimizer}{x^\ast}}

\newcommand\expon[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Exp}_{#1}}}
\newcommand\exponinv[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Log}_{#1}}} 

\newcommand\proj[1]{\newlink{def:projection_operator}{\mathcal{P}_{#1}}}


\renewcommandx*{\PT}[1][1=T, usedefault]{\newlink{def:path_variation}{P_{#1}}}
\newcommandx*{\VT}[1][1=T, usedefault]{\newlink{def:variation}{V_{#1}}}

\newcommand{\Y}{\mathcal{Y}}
\newcommand{\XX}{\mathcal{X}} 

\newcommand\N{\mathcal{N}}

\newcommand\indicator[1]{\newlink{def:indicator_function}{I_{#1}}}


\renewcommand\d{\mathrm{d}}

\newcommand\Tansp[1]{\newlink{def:tangent_space}{T_{#1}}}

\let\oldGamma\Gamma
\renewcommand{\Gamma}[2]{\newlink{def:parallel_transport}{\oldGamma_{#1}^{#2}}}

\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\newlink{def:accuracy_epsilon}{\oldepsilon}}



\let\oldzeta\zeta
\renewcommand\zeta{\newlink{def:zeta_geometric_constant}{\oldzeta}}
\newcommand\zetar{\zeta_{\! R}}
\newcommand\zetad{\zeta_{\! D}}

\let\olddelta\delta
\renewcommand\delta{\newlink{def:delta_geometric_constant}{\olddelta}}

\newcommand\xinit{\newlink{def:initial_point}{x_0}}

\newcommand\CFt{C_t(F)}
\newcommand\CHt{C_t(H)}

\newcommand\Ftt{\tilde{L}_{t}}
\newcommand\Ft{L_{t}}
\newcommand\kappamin{\kmin}
\newcommand\kappamax{\kmax}


\newcommand\set[1]{\{ #1 \}}
\newcommand\setl[1]{\left\{ #1 \right\}}
\newcommand\setsuch[2]{\{ #1 \mid #2  \}}
\newcommand\setsuchl[2]{\left\{ #1 \mid #2  \right\}}

